Multi-antenna Interference Management for Coded Caching

A multi-antenna broadcast channel scenario is considered where a base station delivers contents to cache-enabled user terminals. A joint design of coded caching (CC) and multigroup multicast beamforming is proposed to benefit from spatial multiplexing gain, improved interference management and the global CC gain, simultaneously. The developed general content delivery strategies utilize the multiantenna multicasting opportunities provided by the CC technique while optimally balancing the detrimental impact of both noise and inter-stream interference from coded messages transmitted in parallel. Flexible resource allocation schemes for CC are introduced where the multicast beamformer design and the receiver complexity are controlled by varying the size of the subset of users served during a given time interval, and the overlap among the multicast messages transmitted in parallel, indicated by parameters $\alpha$ and $\beta$, respectively. Degrees of freedom (DoF) analysis is provided showing that the DoF only depends on $\alpha$ while it is independent of $\beta$. The proposed schemes are shown to provide the same degrees-of-freedom at high signal-to-noise ratio (SNR) as the state-of-art methods and, in general, to perform significantly better, especially in the finite SNR regime, than several baseline schemes.

==> abbrev.tex <==
%!TeX root = fibc.tex

% Declaration of the abbreviations
\DeclareAcronym{3G}{
    short = 3G,
    long = third generation,
    list = Third Generation,
    class = abbrev
}

\DeclareAcronym{4G}{
    short = 4G,
    long = fourth generation,
    list = Fourth Generation,
    class = abbrev
}

\DeclareAcronym{5G}{
    short = 5G,
    long = fifth generation,
    list = Fifth Generation,
    class = abbrev
}

\DeclareAcronym{ADMM}{
    short = ADMM,
    long = alternating direction method of multipliers,
    list = Alternating Direction Method of Multipliers,
    class = abbrev
}

\DeclareAcronym{AF}{
    short = AF,
    long = amplify-and-forward,
    list = Amplify-and-Forward,
    class = abbrev
}

\DeclareAcronym{BC}{
    short = BC,
    long = broadcast channel,
    list = Broadcast Channel,
    class = abbrev
}

\DeclareAcronym{BER}{
    short = BER,
    long = bit error rate,
    list = Bit Error Rate,
    class = abbrev
}

\DeclareAcronym{BR}{
    short = BR,
    long = best response,
    list = Best Response, 
    class = abbrev
}

\DeclareAcronym{BS}{
    short = BS,
    long = base station,
    list = Base Station,
    class = abbrev
}

\DeclareAcronym{CB}{
    short = CB,
    long = coordinated beamforming,
    list = Coordinated Beamforming,
    class = abbrev
}

\DeclareAcronym{CoMP}{
    short = CoMP,
    long = coordinated multi-point,
    list = Coordinated Multi-Point,
    class = abbrev
}

\DeclareAcronym{CRAN}{
    short = CRAN,
    long = cloud radio access network,
    list = Cloud Radio Access Network,
    class = abbrev
}

\DeclareAcronym{CSI}{
    short = CSI,
    long = channel state information,
    list = Channel State Information,
    class = abbrev
}

\DeclareAcronym{CU}{
    short = CU,
    long = central unit,
    list = Central Unit,
    class = abbrev
}

\DeclareAcronym{DCP}{
    short = DCP,
    long = difference of convex functions program,
    list = Difference of Convex Functions Program,
    class = abbrev
}

\DeclareAcronym{DE}{
    short = DE,
    long = direct estimation,
    list = Direct Estimation,
    class = abbrev
}

\DeclareAcronym{DF}{
    short = DF,
    long = decode-and-forward,
    list = Decode-and-Forward,
    class = abbrev
}

\DeclareAcronym{DL}{
    short = DL,
    long = downlink,
    list = Downlink,
    class = abbrev
}

\DeclareAcronym{DoF}{
    short = DoF,
    long = degrees of freedom,
    list = Degrees of Freedom,
    class = abbrev
}

\DeclareAcronym{DPC}{
    short = DPC,
    long = dirty paper coding,
    list = Dirty Paper Coding,
    class = abbrev
}

\DeclareAcronym{FDD}{
    short = FDD,
    long = frequency division duplexing,
    list = Frequency Division Duplexing,
    class = abbrev
}

\DeclareAcronym{FIBC}{
    short = FIBC,
    long = fast converging IBC,
    list = Fast Converging IBC,
    class = abbrev
}

\DeclareAcronym{GP}{
	short = GP, 
	long = geometric program,
	list = Geometric Program,
	class = abbrev
}

\DeclareAcronym{GD}{
	short = GD, 
	long = gradient descent,
	list = Gradient Descent,
	class = abbrev
}

\DeclareAcronym{IBC}{
    short = IBC,
    long = interfering broadcast channel,
    list = Interfering Broadcast Channel,
    class = abbrev
}

\DeclareAcronym{i.i.d.}{
    short = i.i.d.,
    long = independent and identically distributed,
    list = Independent and Identically Distributed,
    class = abbrev
}

\DeclareAcronym{JP} {
    short = JP,
    long = joint processing,
    list = Joint Processing,
    class = abbrev
}

\DeclareAcronym{KKT} {
    short = KKT,
    long = Karush-Kuhn-Tucker,
    class = abbrev
}

\DeclareAcronym{LOS} {
    short = LOS,
    long = line of sight,
    list = Line of Sight,
    class = abbrev
}

\DeclareAcronym{LS}{
    short = LS,
    long = least squares,
    list = Least Squares,
    class = abbrev
}

\DeclareAcronym{LTE} {
    short = LTE,
    long = Long Term Evolution,
    class = abbrev
}

\DeclareAcronym{LTE-A} {
    short = LTE-A,
    long = Long Term Evolution Advanced,
    class = abbrev
}

\DeclareAcronym{MAC}{
    short = MAC,
    long = multiple access channel,
    list = Multiple Access Channel,
    class = abbrev
}

\DeclareAcronym{MF}{
    short = MF,
    long = matched filter,
    list = Matched Filter,
    class = abbrev
}

\DeclareAcronym{MIMO}{
    short = MIMO,
    long = multiple-input multiple-output,
    list = Multiple-Input Multiple-Output,
    class = abbrev
}

\DeclareAcronym{MISO}{
    short = MISO,
    long = multiple-input single-output,
    list = Multiple-Input Single-Output,
    class = abbrev
}


\DeclareAcronym{MMSE}{
    short = MMSE,
    long = minimum MSE,
    list = Minimum MSE,
    class = abbrev
}

\DeclareAcronym{MSE}{
    short = MSE,
    long = mean-squared error,
    list = Mean-Squared Error,
    class = abbrev
}

\DeclareAcronym{MU-MIMO}{
    short = MU-MIMO,
    long = multi-user MIMO,
    list = Multi-User MIMO,
    class = abbrev
}

\DeclareAcronym{NLOS} {
    short = NLOS,
    long = non line of sight,
    list = Non Line of Sight,
    class = abbrev
}

\DeclareAcronym{OFDMA} {
    short = OFDMA,
    long = orthogonal frequency division multiple access,
    list = Orthogonal Frequency Division Multiple Access,
    class = abbrev
}

\DeclareAcronym{PSD}{
    short = PSD,
    long = positive semidefinite,
    list = Positive Semidefinite,
    class = abbrev
}

\DeclareAcronym{OTA}{
    short = OTA,
    long = over-the-air,
    list = Over-the-Air,
    class = abbrev
}

\DeclareAcronym{QoS}{
	short = QoS,
	long = quality of service,
	list = Quality of Service,
	class = abbrev
}

\DeclareAcronym{RRH}{
    short = RRH,
    long = remote radio head,
    list = Remote Radio Head,
    class = abbrev
}

\DeclareAcronym{RS}{
    short = RS,
    long = relay station,
    list = Relay Station,
    class = abbrev
}

\DeclareAcronym{SCA}{
    short = SCA,
    long = successive convex approximation,
    list = Successive Convex Approximation,
    class = abbrev
}

\DeclareAcronym{SDP}{
    short = SDP,
    long = semidefinite program,
    list = Semidefinite Program,
    class = abbrev
}

\DeclareAcronym{SNR}{
    short = SNR,
    long = signal-to-noise ratio,
    list = Signal-to-Noise Ratio,
    class = abbrev
}

\DeclareAcronym{SG}{
    short = SG,
    long = stochastic gradient,
    list = Stochastic Gradient,
    class = abbrev
}

\DeclareAcronym{SIC}{
    short = SIC,
    long = successive interference cancellation,
    list = Successive Interference Cancellation,
    class = abbrev
}

\DeclareAcronym{SINR}{
    short = SINR,
    long = signal-to-interference-plus-noise ratio,
    list = Signal-to-Interference-plus-Noise Ratio,
    class = abbrev
}

\DeclareAcronym{SOC}{
	short = SOC,
	long = second order cone,
	list = Second Order Cone,
	class = abbrev
}

\DeclareAcronym{SOCP}{
	short = SOCP,
	long = second order cone program,
	list = Second Order Cone Program,
	class = abbrev
}

\DeclareAcronym{SPMin}{
    short = SPMin,
    long = sum power minimization,
    list = Sum Power Minimization,
    class = abbrev
}

\DeclareAcronym{SSE}{
    short = SSE,
    long = stream specific estimation,
    list = Stream Specific Estimation,
    class = abbrev
}

\DeclareAcronym{SRMax}{
    short = SPMin,
    long = sum rate maximization,
    list = Sum Rate Maximization,
    class = abbrev
}

\DeclareAcronym{TDD}{
    short = TDD,
    long = time division duplex,
    list = Time Division Duplex,
    class = abbrev
}

\DeclareAcronym{UE}{
    short = UE,
    long = user equipment,
    list = User Equipment,
    class = abbrev
}

\DeclareAcronym{UL}{
    short = UL,
    long = uplink,
    list = Uplink,
    class = abbrev
}

\DeclareAcronym{WF} {
    short = WF,
    long = waterfilling,
    list = Waterfilling,
    class = abbrev
}

\DeclareAcronym{WMMSE} {
    short = WMMSE,
    long = weighted minimum MSE,
    list = Weighted Minimum MSE,
    class = abbrev
}

\DeclareAcronym{WMSEMin} {
    short = WMSEMin,
    long = weighted sum MSE minimization,
    list = Weighted sum MSE Minimization,
    class = abbrev
}

\DeclareAcronym{w.r.t.}{
    short = w.r.t.,
    long = with respect to,
    list = With Respect To,
    class = abbrev
}

\DeclareAcronym{WSRMax}{
    short = WSRMax,
    long = weighted sum rate maximization,
    list = Weighted Sum Rate Maximization,
    class = abbrev
}

\DeclareAcronym{ZF}{
    short = ZF,
    long = zero forcing,
    list = Zero Forcing,
    class = abbrev
}


==> commands.tex <==
% ===========================================================================
% File Name: commands.tex
% File Creation Date: 15.6.1995
% Author: Markku Juntti
% Description: Includes useful commands for Latex edition.
% ===========================================================================


% Theorem-like environments
%\newtheorem{defin}{Definition}
%%\newtheorem{theorem}{Theorem}
%%\newtheorem{prop}{Proposition}
%\newtheorem{lemma}{Lemma}
%\newtheorem{corollary}{Corollary}
%\newtheorem{alg}{Algorithm}

% Equations, arrays etc.
\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\ba}{\begin{array}}
\newcommand{\ea}{\end{array}}
\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\eea}{\end{eqnarray}}
\newcommand{\herm}{^{\mbox{\scriptsize H}}}
\newcommand{\sherm}{^{\mbox{\scriptsize H}}}
\newcommand{\tran}{^{\mbox{\scriptsize T}}}
\newcommand{\stran}{^{\mbox{\tiny T}}}

% Sets of numbers
\newcommand{\vbar}{\raisebox{.17ex}{\rule{.04em}{1.35ex}}}
\newcommand{\vbarind}{\raisebox{.01ex}{\rule{.04em}{1.1ex}}}
\newcommand{\R}{\ifmmode {\rm I}\hspace{-.2em}{\rm R} \else ${\rm I}\hspace{-.2em}{\rm R}$ \fi}
\newcommand{\T}{\ifmmode {\rm I}\hspace{-.2em}{\rm T} \else ${\rm I}\hspace{-.2em}{\rm T}$ \fi}
\newcommand{\N}{\ifmmode {\rm I}\hspace{-.2em}{\rm N} \else \mbox{${\rm I}\hspace{-.2em}{\rm N}$} \fi}
%\newcommand{\B}[1]{\ifmmode {\rm I}\hspace{-.2em}{\rm B}^{#1} \else \mbox{${\rm I}\hspace{-.2em}{\rm B}^{#1}$} \fi}
\newcommand{\B}{\ifmmode {\rm I}\hspace{-.2em}{\rm B} \else \mbox{${\rm I}\hspace{-.2em}{\rm B}$} \fi}
\newcommand{\Hil}{\ifmmode {\rm I}\hspace{-.2em}{\rm H} \else \mbox{${\rm I}\hspace{-.2em}{\rm H}$} \fi}
\newcommand{\C}{\ifmmode \hspace{.2em}\vbar\hspace{-.31em}{\rm C} \else \mbox{$\hspace{.2em}\vbar\hspace{-.31em}{\rm C}$} \fi}
\newcommand{\Cind}{\ifmmode \hspace{.2em}\vbarind\hspace{-.25em}{\rm C} \else \mbox{$\hspace{.2em}\vbarind\hspace{-.25em}{\rm C}$} \fi}
\newcommand{\Q}{\ifmmode \hspace{.2em}\vbar\hspace{-.31em}{\rm Q} \else \mbox{$\hspace{.2em}\vbar\hspace{-.31em}{\rm Q}$} \fi}
%\newcommand{\Z}{\ifmmode {\rm\bf Z} \else \mbox{{\rm\bf Z}} \fi}
\newcommand{\Z}{\ifmmode {\rm Z}\hspace{-.28em}{\rm Z} \else ${\rm Z}\hspace{-.28em}{\rm Z}$ \fi}

% Constants
\newcommand{\I}{\mathbf{I}}

% Functions
\newcommand{\sgn}{\mbox {sgn}}
\newcommand{\var}{\mbox {var}}
\renewcommand{\Re}{\mbox {Re}}
\renewcommand{\Im}{\mbox {Im}}

% Bold-face Greek letters
\renewcommand{\vec}[1]{\bf{#1}}     %equation styles %vector/matrix
\newcommand{\vecsc}[1]{\mbox {\bf \scriptsize #1}}
%\newcommand{\itvec}[1]{\mathbf{#1}}     %equation styles %vector/matrix
\newcommand{\itvec}[1]{\mbox {\boldmath $#1$}}
\newcommand{\itvecsc}[1]{\mbox {\boldmath $\scriptstyle #1$}}
\newcommand{\gvec}[1]{\mbox{\boldmath $#1$}}

\newcommand{\balpha}{\mbox {\boldmath $\alpha$}}
\newcommand{\bbeta}{\mbox {\boldmath $\beta$}}
\newcommand{\bgamma}{\mbox {\boldmath $\gamma$}}
\newcommand{\bdelta}{\mbox {\boldmath $\delta$}}
\newcommand{\bepsilon}{\mbox {\boldmath $\epsilon$}}
\newcommand{\bvarepsilon}{\mbox {\boldmath $\varepsilon$}}
\newcommand{\bzeta}{\mbox {\boldmath $\zeta$}}
\newcommand{\boldeta}{\mbox {\boldmath $\eta$}}
\newcommand{\btheta}{\mbox {\boldmath $\theta$}}
\newcommand{\bvartheta}{\mbox {\boldmath $\vartheta$}}
\newcommand{\biota}{\mbox {\boldmath $\iota$}}
\newcommand{\blambda}{\mbox {\boldmath $\lambda$}}
\newcommand{\bmu}{\mbox {\boldmath $\mu$}}
\newcommand{\bnu}{\mbox {\boldmath $\nu$}}
\newcommand{\bxi}{\mbox {\boldmath $\xi$}}
\newcommand{\bpi}{\mbox {\boldmath $\pi$}}
\newcommand{\bvarpi}{\mbox {\boldmath $\varpi$}}
\newcommand{\brho}{\mbox {\boldmath $\rho$}}
\newcommand{\bvarrho}{\mbox {\boldmath $\varrho$}}
\newcommand{\bsigma}{\mbox {\boldmath $\sigma$}}
\newcommand{\bvarsigma}{\mbox {\boldmath $\varsigma$}}
\newcommand{\btau}{\mbox {\boldmath $\tau$}}
\newcommand{\bupsilon}{\mbox {\boldmath $\upsilon$}}
\newcommand{\bphi}{\mbox {\boldmath $\phi$}}
\newcommand{\bvarphi}{\mbox {\boldmath $\varphi$}}
\newcommand{\bchi}{\mbox {\boldmath $\chi$}}
\newcommand{\bpsi}{\mbox {\boldmath $\psi$}}
\newcommand{\bomega}{\mbox {\boldmath $\omega$}}

% Bold italic Roman letters
\newcommand{\bolda}{\mbox {\boldmath $a$}}
\newcommand{\bb}{\mbox {\boldmath $b$}}
\newcommand{\bc}{\mbox {\boldmath $c$}}
\newcommand{\bd}{\mbox {\boldmath $d$}}
\newcommand{\bolde}{\mbox {\boldmath $e$}}
\newcommand{\boldf}{\mbox {\boldmath $f$}}
\newcommand{\bg}{\mbox {\boldmath $g$}}
\newcommand{\bh}{\mbox {\boldmath $h$}}
\newcommand{\bp}{\mbox {\boldmath $p$}}
\newcommand{\bq}{\mbox {\boldmath $q$}}
\newcommand{\br}{\mbox {\boldmath $r$}}
\newcommand{\bs}{\mbox {\boldmath $s$}}
\newcommand{\bt}{\mbox {\boldmath $t$}}
\newcommand{\bu}{\mbox {\boldmath $u$}}
\newcommand{\bv}{\mbox {\boldmath $v$}}
\newcommand{\bw}{\mbox {\boldmath $w$}}
\newcommand{\bx}{\mbox {\boldmath $x$}}
\newcommand{\by}{\mbox {\boldmath $y$}}
\newcommand{\bz}{\mbox {\boldmath $z$}}

